Individual Fairness in Pipelines

It is well understood that a system built from individually fair components may not itself be individually fair. In this work, we investigate individual fairness under pipeline composition. Pipelines differ from ordinary sequential or repeated composition in that individuals may drop out at any stage, and classification in subsequent stages may depend on the remaining "cohort" of individuals. As an example, a company might hire a team for a new project and at a later point promote the highest performer on the team. Unlike other repeated classification settings, where the degree of unfairness degrades gracefully over multiple fair steps, the degree of unfairness in pipelines can be arbitrary, even in a pipeline with just two stages. Guided by a panoply of real-world examples, we provide a rigorous framework for evaluating different types of fairness guarantees for pipelines. We show that na\"{i}ve auditing is unable to uncover systematic unfairness and that, in order to ensure fairness, some form of dependence must exist between the design of algorithms at different stages in the pipeline. Finally, we provide constructions that permit flexibility at later stages, meaning that there is no need to lock in the entire pipeline at the time that the early stage is constructed.

==> sections/extensions.tex <==
%The results presented in this work extend in natural ways to related settings.

\noindent \textbf{Group or statistical notions of fairness.}
Although this work is concerned with individual fairness, many of our results and problematic examples are directly applicable to group or statistical notions of fairness. Our motivating examples apply equally well to group and individual notions of fairness. Extensions of our positive results to group-based notions follow from considering simple metric constructions which capture that similarly qualified members of each group should be treated similarly.\footnote{For example, to satisfy notions like  Conditional Parity \cite{ritov2017conditional}, which captures many popular group-based definitions, one can construct a metric $\D_{parity}$ such that $\D_{parity}(u,v)=1$ for all ``qualified'' members of any protected group and $\D_{parity}(u,v)=0$ for all other pairs. Satisfying individual fairness with respect to $\D_{parity}$ is sufficient to give Conditional Parity, and in fact provides stronger guarantees.
}

\noindent \textbf{Multi-stage pipelines.}
%including multiple cohort selection and scoring steps (Appendix \ref{appendix:generalizingmultiplecohortselectionsteps}),
In Appendix \ref{appendix:generalizingmultiplecohortselectionsteps}, we consider how our framework can be adapted to multi-stage pipelines where the cohort is repeatedly pruned at each stage. For example, a company might have a series of promotions with a compensation decision at each step. We demonstrate that our framework in Section \ref{sec:conditionsforsuccess} can be generalized for Notion 1. For Notion 2, however, we show that the situation is trickier. In practice, however, treating multiple stages of selection as a single combined step and enforcing conditional guarantees only on the final step is still feasible. 

%
% \noindent \textbf{Different metrics at different stages.} Our stylized model considered the case in which the fairness metric was the same for cohort selection and scoring. However, there are many reasonable settings in which different fairness metrics may be applicable at different stages in the pipeline. For example, choosing a project team of talented engineers may be subject to a different metric than promoting an individual to a management position, as the skills needed are somewhat different.


\noindent \textbf{Selecting multiple cohorts.}
Our results also extend in a natural way to selecting multiple cohorts simultaneously (Appendix \ref{appendix:multiplecohortsdetails}).
%In Appendix \ref{appendix:multiplecohortsdetails}, we show that our results extend in a natural way to selecting more than one cohort at a time.
For example, a company opening an office in a new location may need to hire multiple project teams at one time.  We show that some of our robustness guarantees extend naturally to selecting multiple cohorts, either allowing individuals to participate on multiple projects or requiring individuals to be part of exactly one project team.   %In some settings, we may want individuals to be part of exactly one team \mnote{Christina note: ``(For example, selecting several teams at once to open a new office)''}.
%We also demonstrate that some of our mechanisms generalize well to this setting by composing with splitting into teams uniformly at random.
%

\noindent \textbf{Cohorts formed over time.}
%and forming cohorts over longer time periods, e.g., hiring a team over several years (Appendix \ref{appendix:multipleyears}).
In Appendix \ref{appendix:multipleyears}, we give intuition for adapting our framework to handle cohorts formed over multiple years. For example, a team may start from a small set of initial hires and expand over several years as more team members are needed to work on an expanding project. First, we demonstrate that naively enforcing robustness guarantees per-year can be completely at odds with mechanism expressivity, and we then propose that score functions instead be evaluated at coarser time intervals.


==> sections/extraneous-definitions.tex <==
% We first define the swapping mapping formally.
% \begin{definition}
% Let $\mathcal{C}$ be the set of all cohorts of size $k$. Then the \textbf{swapping mapping} is defined by $M_{u,v} = {{|U| - 1} \choose {k-1}}$, and $f_{u,v}(C) = f_{v,u}((C \setminus \left\{u\right\}) \cup \left\{v\right\})$ for all $C \in \mathcal{C}$. 
% \end{definition}

% We state a standard lemma about extensions of functions on metric spaces and we present a proof for sake of being self-contained. 
% \begin{lemma}
% \label{lemma:functioncompletion}
% Let $d$ be a pseudo-metric over $M$ and let $U \subseteq M$. If $f: U \rightarrow [0,1]$ is $\alpha$-Lipschitz w.r.t. $d|_U$, then there exists a function $g: M \rightarrow [0,1]$ such that $g |_U = f$ and that is $\alpha$-Lipschitz w.r.t $d$. 
% \end{lemma}
% \begin{proof}
% Let $g': M \rightarrow \mathbb{R}$ be defined by $g'(x) = \inf_{u \in U} \left\{f(u) + \alpha d(x,u)\right\}$. Observe that $g'|_U = f$. Moreover, observe that for every $\epsilon > 0$, there exists $u^*$ such that: $g'(x) \ge f(u^*) + \alpha d(x,u^*) - \epsilon$. Moreover, we have by definition that $g'(y) \le  f(u^*) + \alpha d(y,u^*)$. Thus:
%  $g'(y) - g'(x) \le f(u^*) + \alpha d(y,u^*) - (f(u^*) + \alpha d(x, u^*)) + \epsilon \le \alpha (d(y, u* - d(x, u^*)) + \epsilon  \le \alpha d(x,y) + \epsilon$. Thus, $g'$ is $\alpha$-Lipschitz w.rt. $d$. Now, we let $g(x) = \min(1, g'(x))$. We see that $g|_U = g'|_U = f$ and $g$ is $\alpha$-Lipschitz w.rt. $d$ since $|g(y) - g(x)| \le |g'(y) - g'(x)|$.   
% \end{proof}



==> sections/fairness-cd.tex <==
\subsection{Fairness in Machine Learning}
\label{sec:fairness}

The embrace and widespread adoption of algorithmic risk prediction tools in the last decade has led to concerns of the introduction and/or reification, entrenchment, and exacerbation of historically unfair treatment of individuals for whom the decisions have life-altering consequences.
These concerns have found their way into news accounts (\cite{Dastin}) and general interest books \cite{mathbabe16,KR19}. Even when these algorithms are deployed in domains subject to regulation, it appears that existing regulation is poorly equipped to deal with this issue (\cite{SullScott}). 

 This is in part because most documented examples of systemic algorithmic misbehavior are {\em side-effects} of the standard methodology of machine learning: blind optimization of a narrow objective function.
This methodology results in models that may be exceedingly good as measured according to the objective function for which they were optimized.  But ``garbage in, garbage out'' applies in fairness as everywhere else: do the features in the data have the same meanings across different demographic groups?  Are the proxies optimized for in the obvjective function equally expressive across groups?  Dos the objective function appropriately capture variation within all groups?

Fixing this requires new science: what \emph{precisely} constitutes unfairness, how can it be avoided by modifying the standard machine learning training pipeline -- including the choice of features to collect and outputs to be measured, and what are the consequences and tradeoffs involved in doing so? It also requires rethinking legal and regulatory frameworks used to govern decision-making that is increasingly automated.  

\subusbsection{Foundations of Algorithmic Fairness.}
From its inception, the field of algorithmic fairness exhibited a tension between notions of {\em group fairness} notions, which define the problem in terms of comparisons between statistics across a small number of disjoint ``protected'' demographic groups, and {\em individual fairness}, now also known as {\em metric fairness}, which captures the notion that individuals that are similar, for a given classificatin or scoring task, should be treated similarly~\cite{awareness}.  Group fairness conditions are immediately actionable and easy to check (although~\cite{NeilWinship} raises compelling challenges to most standard benchmark tests, group notions can be ``gerrymandered''~\cite{awareness,KNRW18}; natural group fairness desiderata cannot coexist~\cite{Chouldechova,KMR}), while individual fairness requires a metric specifying for each pair of individuals, their (dis)similarity for the task in question.  {\em Finding} the metric is a technical hurdle (although we mention a recent tantalizing breakthrough below).

The tension between clinical prediction, which uses individual-level traits, and actuarial prediction, which uses group-level traits, has animated penology since the 1920's~\cite{burgess1928prediction}, 
psychology since the 1950's~\cite{meehl1954clinical}, 
legal scholarship since the 1970's~\cite{Underwood1979,Schauer}, 
and statistics since the 1980's ~\cite{dawid2017individual}. 
This tension persists in artificial intelligence:  
a prominent application of fairness research is in individual risk prediction, {\it e.g.}, ``What is the chance that a given individual will commit a violent crime in the next two years?'' But what is the meaning of ``individual risk'' and  ``chance'' in this context?  Can group traits provide fair estimates of individual chance, and if so, which groups should be considered?  

%Between the extremes of group-based and individual notions of fairness,
Definitions of fairness based on statistical requirements on the treatment of (potentially large numbers of) {\em arbitrarily intersecting} sets, not only (finally!) aim to address intersectional issues and bridge the gap between meaningless and conflicted group guarantees and insufficiently actionable individual guarantees~\cite{HKRR18,KNRW18}.

Given a good definition of fairness, the next goal is to understand how fairness guarantees compose: if an algorithm is fair when executed once, is it fair when run many times?  Are systems composed of fair parts also fair as a whole?  More generally, how do fairness guarantees behave under composition?  We need to choose meaningful definitions that compose well.  

\paragraph{Individual (aka Metric) Fairness} was defined by Co-PI Dwork and collaborators in the first theoretical treatment of algorithmic fairness~\cite{awareness}; it provides a powerful framework for fair classification and scoring in a variety of contexts~\cite{DI2018,ChawlaIJ19,DworkIJ2020,RothblumYona,Stanford2,Penn2}.  As noted, finding the metric may be hard.
In a tantalizing breakthrough, by combining insights from human-computer interaction (HCI) and learning theory, Co-PI Dwork's student Christina Ilvento showed how to obtain an approximation of a metric from a human arbiter, who may have an excellent understanding of the degree of (dis)similarity, for a given classification task, between pairs individuals but cannot articulate an algorithm~\cite{Ilvento}.  Ilvento distinguishes between two types of queries to the arbiter: difficult queries ask for absolute distances between individuals, while easy queries ask which of two individuals is closer to a third. Under very mild assumptions Ilvento's method requires only a constant number of difficult queries and $O(n \log n)$ easy queries, where $n$ is the number of individuals in the universe.  (One can work with a sample and generalize via the techniques in~\cite{RothblumYona} to obtain a relaxed notion of approximate metric-fairness.) Ilvento's work suggests that metric fairness may be more actionable than was previously thought. A natural next question is whether multiple arbiters, each of which may be knowledgeable about different subpopulations, might divide up the work.  This will be the subject of an undergraduate research project supervised by Co-PI Dwork this semester.

Most research on fairness treats the ``one-shot'' case.  Co-PI Dwork and Ilvento have shown that both individual/metric and group fairness can behave very badly under composition~\cite{DI2018}, and that different kinds of composition can have very different behaviors. For example, in {\em competitive} composition two advertisers, say a grocery delivery service and a technical jobs advertiser, compete for a single banner slot on a webpage.  Even if each advertiser is perfectly individually fair, the grocery delivery service targeting new parents may consistently outbid the tech jobs advertiser, resulting, over time, in worse employment and compensation opportunities for the parent.  Simple solutions provide fairness even in this competitive scenario, but leave a lot of money on the table~\cite{DI2018}.  (Similar problems also arise with group fairness.)  This scenario was further investigated in~\cite{CIJ20,KKRY19}.

Dwork and Ilvento also considered sequential composition and {\em cohort} selection, in which the number of positively classified individuals is fixed in advance ({\it e.g.}, due to capacity or budget constraints).  These two concepts come together in the construction of fair pipelines. {\em Pipelines} differ from ordinary sequential composition in that individuals may drop out of consideration at any stage~\cite{Bower17,DIJ20}.  
Pipelines are common: many data-driven systems consist of a sequence of ``cohort selection,'' or filtering steps, followed by a decision or scoring step.  For example, a hiring pipeline might consist of an automated resume screening program followed by human review followed by interviews and a hiring decision. 
The starting point for \cite{DIJ20} is an observation that, unlike other sequential classification settings in which the degree of unfairness of multiple fair steps degrades gracefully, the degree of unfairness in cohort-based pipelines can be arbitrary, even in a pipeline with just two stages. For example, consider hiring a team, followed by a bonus award stage in which compensation depends fairly on ranking within the team. Although the team selection may be fair in the sense that similarly qualified candidates have similar chances of being chosen for the team, an individual's ranking critically depends on the \textit{other members of the team}. Being compared fairly to other members of the cohort simply doesn't imply fairness of the entire pipeline, as the competitive landscape can vary between similar individuals.  
Dwork and her collaborators show that naive auditing is unable to uncover systematic unfairness and that, in order to ensure fairness; and that some form of dependence must exist between the design of algorithms at different stages in the pipeline; and they provide constructions that permit flexibility at later stages, meaning that there is no need to lock in the entire pipeline at the time that the early stage is constructed.  They further consider many generalizations of basic the scenario.  

However, many questions remain open; in some of these it is not even clear how to \texit{define} fairness.  For example:  \cite{DIJ20} does not take into account the preferences of individuals during the team formation process;
Cohorts may interact in the future, {\it e.g.}, the top person from each team is promoted to management, among whom executives are chosen; 
there is no complete characterization of the communication complexity between stages.

\paragraph{Multi-Group Fairness Notions: Classification}
Group fairness notions are easily subverted -- requirements to advertise equally to blacks and whites are subverted by a racist steak house restauranteur advertising to black vegetarians and white omnivores~\cite{awareness} or ``fairness gerrymandering''~\cite{KNRW18} that equalizes false positive rates across both gender (men, women) and racial (white, black) groups but has the maximum possible false positive rate differential between {\it e.g.} white men and black women. 

In preliminary work, co-PIs Kearns, Roth and colleagues \cite{KNRW18} offer a partial mitigation to this problem, by asking for statistical fairness constraints that hold not only over a small number of coarsely defined groups, but over exponentially many or even infinitely many finely defined \emph{subgroups} implicitly defined by a class of group indicator functions $\mathcal{G}$. If $\mathcal{G}$ represents the class of  conjunctions, for example, this corresponds to asking for \emph{intersectional} fairness constraints --- equalizing false positive rates (or positive predictive value) not just amongst men, black people, disabled people, etc, but also across groups defined by the intersections of these attributes, like black disabled men. As we show, so long as the VC-dimension of $\mathcal{G}$ is bounded, the \emph{statistical} problem of imposing these fairness constraints is easy: if they are satisfied in-sample, then they will be satisfied out of sample, given a sufficiently large sample. The computational problem is more interesting. What we show is that for a broad family of statistical fairness constraints, the problem of learning the most accurate (distribution over) classifiers in $\mathcal{H}$ subject to satisfying subgroup fairness over every group implicitly defined by $\mathcal{G}$ can be reduced to a small number of \emph{unconstrained} learning problems over $\mathcal{H}$ and $\mathcal{G}$ respectively. Hence, if we have good learning heuristics for $\mathcal{H}$ and $\mathcal{G}$ (such as e.g. support vector machines and logistic regression for linear threshold functions, and neural networks for more complex families), they can be used to solve the fair learning problem as well. We call algorithms of this sort ``oracle efficient'' because they are efficient reductions to standard learning ``oracles'' for which we have practical heuristics. This has proven to be a fruitful design methodology.

We intend to continue to exploit the framework of oracle efficiency to investigate other notions of fairness that have meaningful guarantees. For example, we have recently used this framework to elicit the subjective ``fairness judgements'' of individuals that can play the role of the otherwise hard-to-pin-down metric in individual fairness and optimize subject to the implied constraints \cite{JKNRSW19}. We also used this methodology to optimize subject to an individual fairness constraint that makes sense in settings in which individuals are subject to an entire {\em distribution over classification problems}, rather than a single classification problem \cite{KRS19}. In such settings, one can define ``false positive rates'' and other traditional statistical measures of fairness for particular individuals, by defining the ``rate'' to be over the randomness of the problem distribution, rather than averaging over people. We can then enunciate and enforce ``individual'' fairness constraints that require that false positive rates (e.g.) be equalized across people, which removes the need to pre-specify protected groups \cite{KRS19}.

\paragraph{Multi-Group Fairness Notions: Scoring}
A {\em scoring function} maps individuals to real-valued scores, often (and throughout this section) in $[0,1]$ and often interpreted as probabilities of a particular binary outcome, for example, the chance of rain.  The traditional notion of calibration for scoring functions requires, roughly speaking, that among those assigned a score of $v\in[0,1]$ a $v$ fraction experience positive outcomes,{\it i.e.}, it rains on one quarter of the days assigned the score~0.25.

Hebert-Johnson {\it et al.}, independently of~\cite{KNRW18} and at the same time, proposed {\em multi-calibration} for scoring functions:  for a pre-spectified collection of arbitrarily intersecting sets, multi-calibrated predictors enjoy the classical statistical notion of calibration on each set simultaneously~\cite{HKRR18}.  The sets in the collection simultaneously serve two purposes: they define demographic groups, so that multi-calibration demands calibration for each demographic group in the collection, and they provide characterizations of individuals who may be comparable for the scoring task at hand. Crucially, \cite{HKRR18} proposed that the definition of the sets be complexity-theoretic, for example, the collection of all sets that can be defined by a decision tree of height~6. This ``automatic'' naming ensures calibration for all demographic groups that can be so recognized. Thus, the job of advocating for a victimized group does not require the members of the group -- who may have internalized negative societal judgements and not even realize the extent to which they are the victims of discrimination -- to demand that the group be recognized and protected and that the scoring function be calibrated on this group: if the group has a concise description then the function will be calibrated automatically for this set. 
The machine-learning algorithms developed in~\cite{HKRR18} operate on historical outcomes data, where the labels are in $\{0,1\}$.  Thus, there are no scores in the training data, but, remarkably, the algorithms nonetheless produce multi-calibrated scoring functions.

\paragraph{Multi-Group Fairness Notions: Ranking}
Scrutiny of the modeling assumptions for risk scoring, while technically impeccable, surface deep philosophical questions about the notion of individual risk.  We return to this point below.  For now, let us simply assume that individuals are imbued with individual probabilities of a positive outcome. 
Unpaid Collaborator Wallach has noted that, in industry, the foci on classification and scoring are misplaced, and that the key problem in practice is ranking.   
In~\cite{DKRRY19} Co-PI Dwork and collaborators generalized the multi-set approach to fairness in~\cite{KNRR18,HKRR18} to define definitions of fairness for {\em ranking} individuals. 
Rankings introduce unique challenges, as fairly ranking an individual (or even considering average rankings for members of a specific demographic group) requires understanding their qualities and qualifications in relation to those of others. In~\cite{DKRRY19} Co-PI Dwork and her collaborators studied the problem of generating a fair ranking function from historical (binary) outcomes data.
As in multi-calibrated scoring, the ranking algorithms of Dwork {\it et al.} train on data with binary labels: no examples of real-valued scores or ranks are seen in training.  In addition to obtaining ``Occam's razor'' conditions that allow the learning of accurate ranking functions, Dwork {\it et al.} proposed (1) fairness requirements based on historical binary outcomes training data, and (2) fairness requirements based on a ``catalog of evils'' describing poor relative treatment of groups.  In each category they defined a (short) hierarchy, and then showed equivalence of the top levels.  Moreover, multi-calibrated predictors yield this top-level construct, highlighting the value of multi-calibration as a fairness notion.  

Viewing the training data as the evidence, for a given dataset and collection ${\cal C}$ of sets, there may be many evidence-consistent scoring functions that are multi-calibrated (and provide fair ranking functions) with respect to~${\cal C}$.  This provides the algorithm designer with the ability to skew the function in a way that cannot be detected on the sets in ${\cal C}$.  Co-PI Dwork and collaborators introduce the notion of {\em latitude}~\cite{DKRRY19}, which captures the extent to which ${\em C}$ (and the training data) pin down the outcomes for a set~$S \in {\cal C}$.  In an ongoing exploration of this property that have been investigating the difficulty of computing latitude, which boils down to understanding the maximal extent to which multi-calibrated predictors (or more generally, predictors in any given class ${\cal K}$ can differ writh respect to some fairness condition $q(\cdot)$ on predictors (or ranking functions), for example, $q_S(p)$ might denote the average score assigned by predictor $p$ to members of $S$, or the fraction of members of $S$ whose score is above a certain threshold.  It quickly becomes apparent that latitude cannot be computed from a sample, leading to the formulation of various constrained versions of latitude.  This work is in its early stages, and we have obtained preliminary results for the set of linear predictors.

\paragraph{Individual Risk}
Another basic issue confronting notions of individual fairness is how to interpret probabilities. The outputs of {\em risk assessment tools}, or {\em scoring functions}, are often described as probabilities: What is the probability that the tumor $T$ will metastasize under a given course of treatment?  What is the probability that this individual will click on an ad, or commit a violent crime?
But what does ``probability'' mean for a non-repeatable event?  For example, suppose we have two studies of tumors.  One study examines tumors with specific genetic markers and reports that $40\%$ of these metastasize.  The second study examines tumors with other markers and reports that $70\%$ metastasize.  Suppose the tumor $T$ shares the characteristics of both studies.  What should we conclude: $40\%$ or $70\%$?  Or perhaps neither: what if the second study also has a metastasis rate of $40\%$?  

Inferring {\em individual} risks from statistical information about groups is tricky (at best!), and yet AI is routinely called upon to perform such deductions. When fairness is concerned, the question of ``why did you view me as part of this group rather than another, less risky, group?" is especially critical. At a minimum, when performing individual predictions, we should be able to understand their meaning and their guarantees in terms of the potential for unfair discrimination.

The search for a rigorous approach to individual probabilities dates back at least as far as the early 1980s. Indeed, in his recent survey paper ``On Individual Risk,'' Philip Dawid examines nine explications of the term ``individual risk'' based on a variety of interpretations of ``probability.''
(Dwork will co-teach a graduate reading course with Prof.\,Joseph Blitzstein, from the Harvard Statistics department, on the literature on individual probabilities in Fall, 2020.) Co-PI Dwork and collaborators have recently proposed defining individual risk through the lens of complexity theoretic-randomness, drawing an analogy between the sets used in multi-calibration and statistical tests used in the theory of pseudo-randomness.    
\cd{Add a sentence on what we know at this point.}




\paragraph{The Universal Achilles Heel: Features and Proxies}
%As proved in~\cite{HKRR18} and~\cite{KNRW18}, the difficulty of ensuring multi-set accuracy depends on the agnostic learnability of the collection of sets, which can present challenges when the set is large.  However, even when there are no computational problems, at least three fairness problems remain: with the data, with the collection of sets, and with the fairness goals.  We briefly describe each of these.  

Consider college appications, and suppose one of the attributes is the number of advanced placement (AP) classes that an applicant has completed with a grade of ``B'' or better.  The {\em meaning} of the value reported may vary with the wealth of the school district of the applicant: a wealthy high school may offer a wide range of AP classes, while an economically disadvantaged school may offer only a handful or even none.  More broadly, in ``Talent is Everywhere,'' SP Danielle Allen has proposes a method of college admission decision-making based on the belief that talented students are geographically distributed.  In analogy, we expect that ``variability is everywhere,'' in the sense that both talent and lack of talent are distributed among different demographic groups.  The data must contain features sufficient for capturing this variability.  

Eubanks points out another source of bias in seemingly neutral data fields, still in the context of fiedling calls to a child abuse hotline: the availability of medical records for individuals obtaining benefits from the state, including Medicaid or state-funded substance abuse programs, and the unavailability of these data for wealthy individuals.

Another known problem is the choice of proxy variables for outcomes, for example, the use of a second call to the hotline within a fixed time frame as a proxy for child neglect or abuse~\cite{Eubanks}, which is more likely to occur in an urban area than in a rural one.


These concerns must be formalized so that data and algorithms can be meaningfully tested.  These efforts are well under way for multi-calibration; this effort needs to be sustained and extended to other classes of classifiers and predictors.

%For example, assuming that variability is present in a set $S$, we should demand such variability in any fair scoring function.  Since the collection ${\cal C}$ of sets in a multi-calibrated scoring function also provides characterizations of individuals who may be comparable for the scoring task at hand, we are concerned with the question of evaluating the collection ${\cal C}$ given the features in the data: A scoring function that distinguishes talented students from untalented students in one demographic group but not in others is underserving the latter populations.  

Finally, the accuracy criteria require the scoring functions to capture the world as it is, in which people are routinely disadvantaged and degraded based on immutable and irrelevant traits.  There is no guidance on how and when to adjust scores to reflect an ideal world, in which each individual is supported to reach her full potential.  Even stating the goal is a major challenge, but this is precisely the kind of question the interdisciplinary strength of the proposed Institute will help us to attack.
%
% An interesting question is whether we can bring to bear the techniques of Daskalakis {\it et al.} on estimating efficient statistics from truncated samples~\cite{DGTZ18}.
%https://arxiv.org/pdf/1809.03986.pdf

%Despite the explosion of research in algorithmic fairness and the many directions set out in this proposal, there remains much foundational work to be done.  Even if we cannot find satisfying, actionable definitions for very wide settings, there may be more restricted settings (like the many-problem setting of \cite{KRS19}) that are amenable to meaningful, special-purpose definitions. 



%****
\cd{THIS IS AS FAR AS I GOT.}
\cd{The next section should include text about Chen and Hu (don't forget to cite Hardt's related work).}


\paragraph{Feedback Loops and Long Term Effects} A common feature of many of our motivating applications, both at the Federal Reserve Bank of Philadelphia and at the First Judicial District of Philadelphia is that machine learning is deployed to predict the behavior of people --- for example, whether someone will repay a loan, or whether they will commit a crime. Moreover, these predictions are typically used to determine an intervention, e.g. to extend a loan or grant bail. In cases like this, the outcome of the prediction (and the incentives engendered by the machine learning algorithm making the predictions) can in turn \emph{change} people's behavior, resulting in feedback loops. This effect has been documented in the context of bail \cite{Cowgill} and predictive policing (by SP Lum \cite{Lum}). 

The existing tools of machine learning are ill-suited to predicting the long-term effects of deploying a particular algorithm, because the bulk of learning theory for classification problems is predicated on the assumption that the environment that the algorithm is operating in is \emph{static}. Co-PIs Kearns, Roth, and collaborators have used the tools of reinforcement learning to study various fairness constraints in dynamic settings \cite{JJKMR17}, but while reinforcement learning in principle can model the kinds of feedback loops present in real systems, the framework seems too general (and hence requires too many rounds of experimentation) to be able to apply in most real-world systems of interest. Moreover, individual behavior does not respond in \emph{arbitrary} ways to the introduction of new algorithmic systems and incentives, but typically in rational ways --- and hence we can apply tools from game theory, economics, and the social sciences to try and predict the equilibrium effects of local changes in AI systems. 

%Thus, providing ex ante predictions is no less important than ex post evaluations for situations with feedback loops.  Measuring the effect of an algorithm on an outcome is inherently difficult because decisions made (or influenced) by an algorithm may have happened identically in the absence of the algorithm. Randomized controlled trials would be a natural way to assess such effects, but randomization may be repugnant in some applications of interest and requires smart experimental design. Absent randomized controlled trials, the regression discontinuity method ("RD" (\cite{LeeLem}) is a useful tool for measuring causal impact. Many machine learning applications make use of a continuous prediction (or score) with a decision threshold for an intervention, and the RD method estimates causal effects by looking at examples slightly below and above this threshold (assuming they are otherwise essentially identical). Papers that have used RD to study the causal impact of algorithms include (\cite{Cowgill}), (\cite{Berk}), (\cite{anderson2013steering}), and (\cite{Stevenson}).

We have already made some progress in this direction. The field of fairness in machine learning has no agreed upon definition of fairness. In fact, we know from \cite{KMR16} and \cite{Chou17} that there are  multiple notions of statistical fairness which are individually reasonable but are mutually incompatible. For example, if we believe that it is the errors of a classifier that lead to harm, we may want to equalize false positive rates and false negative rates across multiple population groups. Or, if we believe that it is important that the actionable content of a prediction not depend on individuals' protected attributes, we may want to equalize positive predictive value across groups. But we cannot generally equalize all three \cite{KMR16,Chou17}. This has led to debates about which --- if any --- of these notions is appropriate to use in particular circumstances, and little concrete guidance about which to prefer. An especially salient use case is criminal recidivism prediction, in which  ``risk scores'' are computed to estimate the probability that an individual will commit a crime again in the next 18 months if released on parole. These debates, however, have taken place imagining that the environment is static, in the sense that policy decisions made will have no effect on the environment in which a classifier is being deployed. We propose, instead to apply game theoretic modeling to predict how behavior will change in response to deployed machine learning models, and to use the resulting predictions to study the equilibrium effects of imposing various fairness constraints. Our recent work (by institute members Roth, Kannan, and Vohra, together with collaborators) has shown that  doing so radically changes the terms of the debate in this setting. Deploying machine learning models that equalize false positive rates turns out to set incentives that results in exactly minimizing crime rates. Deploying machine learning models that satisfy other proposed notions of fairness, like equalizing positive predictive value, or applying identical thresholds on ``calibrated'' risk scores does not.  In terms of a policy pronouncement, this corresponds to committing \emph{not to condition on group membership when computing risk scores}, even when group membership is statistically informative. This is because conditioning on information that an individual has no ability to change (group membership) has a perverse effect on incentives. This illustrates the importance of considering the effects that a particular deployed AI/ML system will have on  behavior when debating different technical notions of fairness.

A focus of the proposed Institute is to apply the tools of economic modeling to predict the long-term impacts of deployed machine learning interventions more broadly. This will utilize the expertise in game theory and social sciences of institute members Chen, Kearns, King, Roth, Vohra, and Watts. Our investigations will be grounded in the many concrete-use cases represented in the data of our government partner institutions. This includes large datasets of granular consumer credit, real estate and mortgage transactions held by  the Federal Reserve Bank of Philadelphia. --- which are each domains in which policy interventions can be expected to have important effects on consumer behavior, and the criminal justice applications relevant to the First Judicial District of Philadelphia. This work will be mediated by our existing collaborations between PI Kearns and the Federal Reserve Bank of Philadelphia, and SP Lum and the First Judicial District of Philadelphia.  
%Going forward, we hope to generalize this result so as to be able to give more robust guidance in a wider range of circumstances. In particular, our current setup is limited to the setting in which 1) signal distributions are identical across populations conditional on the decision to commit a crime, and 2) signal distributions are independent of outside option values, conditional on the decision to commit a crime. Neither of these conditions is fully met in practice. We will investigate whether there are general, weak conditions under which the optimal solution has a false positive rate differential that is \emph{smaller} than the myopic solution. We will also investigate richer models, in which detection rates are a function of the decisions of individual police officers, who may have their own incentives that need to be managed. Finally, we will investigate this framework as it relates to individual notions of fairness \cite{awareness,JKMR16,KNRW18,HKRR18,GJKR18,KRS19,JKNRSW19}.


%Equalizing false positive and false negative rates in this setting has been criticized because it usually requires \emph{disparate treatment}, in the sense that to achieve it, one must apply a \emph{different threshold} to individual risk scores for different groups. Indeed, simply applying the \emph{same} threshold to each individual (current practice) has been proposed as an important aspect of fairness \cite{CPFGH17}.

%The challenge is to model the feedback loop when designing metrics. Further, can we understand when a deployed system will still be able to be used for inference on cause and effect?
%f) The `insufficiently' diverse research teams hypothesis, is often cited as a reason for unfair machine learning algorithms. Yet, we have no systematic documentation of the effects of biased programmers or the effects of diverse AI workforce on the outputs created by practitioners.


\subsubsection{Fairness in AI}


\paragraph{Private Synthetic Data and Unfairness} 
Differentially private algorithms provide the same worst-case guarantees for every individual in the database.  However, the {\em impact} of inaccuracies introduced by differential privacy will depend on how the data are used, and this impact may be unequally distributed across demographic groups, as the uses will differ across groups. This can exacerbate inequities in e.g. the distribution of federal resources. Of particular concern to us is the enforcement of the Voting Rights Act. 

Of special importance in the American Community Survey data is information about the citizen voting age population, which, when combined with the decennial census data, yields the breakdown by race and ethnicity of this population. These data play a central role in enforcement of the Voting Rights Act.

Plaintiffs in a Voting Rights Act case wish to show that it would be possible to draw another district in which it it is possible to elect a candidate preferred by the members of their group (which might be a coalition, where no single minority group is able to elect its preferred candidate alone; while such districts have been approved by lower courts, the Supreme Court has not addressed whether the Voting Rights Act can require coalition districts).  The statistical problem of determining ``ability to elect'' based on demographic data, election turnout, and election results gave rise to the field of {\em ecological inference}, pioneered by SP Gary King~\cite{ei}. This is used to determine how minority-heavy a district has to be to counted as a {\em minority-opportunity} district, that is, a district in which minority voters are consistently able to elect their preferred candidates.  Thus, a ``minority opportunity'' district can be majority-minority or not; it all depends on turnout, voting patterns, racial polarization, and so on.
 
This gives rise to the problem of privately generating synthetic data and developing new techniques for ecological inference that ``play well'' with the synthetic data, meaning, they would have outcomes that are likely to match the outcomes of non-private ecological inferences.  Dwork and King will lead this effort.


\paragraph{Human-in-the-Loop AI Systems} Despite a great deal of hype and concern, there are still very few high stakes decisions that are made \emph{solely}  by algorithms without human input. For example, while risk score models are used to inform bail and parole decisions in many states, these decisions are still ultimately made by human judges. Although resume screening and churn prediction tools are used by HR departments, final employment and compensation decisions continue to be made by human hiring managers. Despite this, the vast majority of the existing technical literature on ``fairness in machine learning'' operates under the assumption that the deployed machine learning algorithms are directly involved in decision making. This is implicit, for example, when fairness constraints are expressed directly in terms of (e.g.) the false positive rates of a deployed classifier. Even if we believe that it is the individuals corresponding to false positives who bear the cost of mistaken predictions (as we might e.g. in parole decisions), we should want to equalize the false positive rates \emph{of the actual, realized decisions} and not of the classifier itself. 

If what we really aspire to do is affect outcome-based notions of fairness, then we need to understand how human decision makers change their behavior in the presence of machine-learning derived recommendations, and design machine learning based tools with this interaction in mind. We (SP Chen and collaborators \cite{GC19a,GC19b}) have already begun an empirical investigation of this question, which we plan to continue. We also intend to begin a theoretical investigation of the question using established tools of economic theory. In particular, the question of how to design algorithmic recommendations to help achieve a goal defined on the resulting human decision making is closely tied to two classic problems in economics: the principle agent problem, and the problem of Bayesian Persuasion \cite{KG11}. Bayesian Persuasion in particular studies the problem of how to design an informative signal to a rational Bayesian agent who will make a decision so as to maximize her own expected utility function over her posterior belief about the true state of the world, conditioned on the signal. In fact, the original paper \cite{KG11} grounds the problem in a criminal justice context, in which a judge --- who simply wants to make the correct determination of guilt or innocence for an accused party --- receives a signal from a prosecutor, who knows the ground truth, but wants to obtain a conviction no matter what. The problem is substantially more complicated in our context, in which a risk prediction algorithm has only a noisy signal about the ground truth, and has a more complicated goal: perhaps (e.g.) to equalize the human judge's false positive rates across different demographic groups. Nevertheless, this connection to an established economics literature, together with the economics expertise on our team (Chen, Kearns, Roth, Vohra) make this a promising direction to explore fairness constraints that can feasibly be enforced in machine learning pipelines that attempt to obtain a goal defined on the whole system (including the human decision maker), and not merely myopically on the predictions of the algorithm itself.  

\iffalse
\ar{Section in progress before here. (Old text follows)}

Few consequential decisions are made by algorithm alone, yet the technical literature focuses on `fairness' at the algorithmic level only. An algorithm's output, is but one among many inputs to a human decision maker. Unless the decision maker strictly follows the recommendation of the algorithm, any fairness requirements satisfied by the algorithm's output need not be satisfied by the actual decisions. Thus, it is important to understand how human decision making interacts with the algorithm's output. Examples of questions that need to be resolved:
\begin{enumerate}
\item How do human decision makers interpret and integrate the output of algorithms?
\item When they deviate from the algorithmic recommendation is it in a systematic way?
\item What role do institutional incentives for decision makers play in how they interpret the output of algorithms?
\item What can one say about the design of an algorithm that results in fair (fairer?) decisions by the human, which complements human decision making?
\item What aspects of a decision process should be handled by an algorithm and what by a human to achieve desired outcomes?
\end{enumerate}
\fi 



\paragraph{Actionable Notions of Individual Fairness}
The algorithmic fairness literature largely considers \emph{group} notions of fairness, which fix a small number of ``protected groups'', and then ask that some statistic of the classifier be approximately equalized across these groups. These are popular in large part because they are immediately actionable, but have a number of well-known shortcomings related to the fact that they are constraints that bind only over coarse averages rather than on individual data points \cite{awareness}. As a canonical example, consider the phenomenon highlighted by \cite{KNRW18} under the name ``fairness gerrymandering'': a solution that equalizes false positive rates across both gender (men, women) and racial (white, black) groups may still have the maximum possible false positive rate differential between e.g. white men and black women. More generally, optimizing an objective function subject to coarse constraints can still ``pack'' the unfairness into structured subgroups.

In preliminary work, co-PIs Kearns, Roth and colleagues \cite{KNRW18} offer a partial mitigation to this problem, by asking for statistical fairness constraints that hold not only over a small number of coarsely defined groups, but over exponentially many or even infinitely many finely defined \emph{subgroups} implicitly defined by a class of group indicator functions $\mathcal{G}$. If $\mathcal{G}$ represents the class of  conjunctions, for example, this corresponds to asking for \emph{intersectional} fairness constraints --- equalizing false positive rates (or positive predictive value) not just amongst men, black people, disabled people, etc, but also across groups defined by the intersections of these attributes, like black disabled men. As we show, so long as the VC-dimension of $\mathcal{G}$ is bounded, the \emph{statistical} problem of imposing these fairness constraints is easy: if they are satisfied in-sample, then they will be satisfied out of sample, given a sufficiently large sample. The computational problem is more interesting. What we show is that for a broad family of statistical fairness constraints, the problem of learning the most accurate (distribution over) classifiers in $\mathcal{H}$ subject to satisfying subgroup fairness over every group implicitly defined by $\mathcal{G}$ can be reduced to a small number of \emph{unconstrained} learning problems over $\mathcal{H}$ and $\mathcal{G}$ respectively. Hence, if we have good learning heuristics for $\mathcal{H}$ and $\mathcal{G}$ (such as e.g. support vector machines and logistic regression for linear threshold functions, and neural networks for more complex families), they can be used to solve the fair learning problem as well. We call algorithms of this sort ``oracle efficient'' because they are efficient reductions to standard learning ``oracles'' for which we have practical heuristics. This has proven to be a fruitful design methodology.

We intend to continue to exploit the framework of oracle efficiency to investigate other notions of fairness that have meaningful guarantees. For example, we have recently used this framework to elicit the subjective ``fairness judgements'' of individuals that can play the role of the otherwise hard-to-pin-down metric in the metric (individual) fairness approach of co-PI Dwork \cite{awareness} and optimize subject to the implied constraints \cite{JKNRSW19}. We also used this methodology to optimize subject to an individual fairness constraint that makes sense in settings in which individuals are subject to an entire distribution over classification problems, rather than a single classification problem \cite{KRS19}. In such settings, one can define ``false positive rates'' and other traditional statistical measures of fairness for particular individuals, by defining the ``rate'' to be over the randomness of the problem distribution, rather than averaging over people. We can then enunciate and enforce ``individual'' fairness constraints that require that false positive rates (e.g.) be equalized across people, which removes the need to pre-specify protected groups \cite{KRS19}.

Hebert-Johnson {\it et al.}, independently of~\cite{KNRW18} and at the same time, proposed {\em multi-calibration} for scoring functions.  For a pre-spectified collection of arbitrarily intersecting sets, multi-calibrated predictors enjoy the classical statistical notion of calibration on each set simultaneously~\cite{HKRR18}.  The sets in the collection simultaneously serve two purposes: they define demographic groups, so that multi-calibration demands calibration for each demographic group in the collection, and they provide characterizations of individuals who may be comparable for the scoring task at hand. Crucially, \cite{HKRR18} permit the definition of the sets to be complexity-theoretic, for example, the collection of all sets that can be defined by a decision tree of height~6. This "automatic" naming ensures calibration for all demographic groups that can be so recognized. Thus, the job of "sticking up for" a victimized group does not require the members of the group -- who may have internalized negative societal judgements and not even realize the extent to which they are the victims of discrimination -- to demand that the group be recognized and that the scoring function be calibrated on this group: if the group has a concise description then the function will be calibrated automatically for this set. 

As proved in~\cite{HKRR18} and~\cite{KNRW18}, the difficulty of ensuring multi-set accuracy depends on the agnostic learnability of the collection of sets, which can present challenges when the set is large.  However, even when there are no computational problems, at least three fairness problems remain: with the data, with the collection of sets, and with the fairness goals.  We briefly describe each of these.  

Consider college appications, and suppose one of the attributes is the number of advanced placement (AP) classes that an applicant has completed with a grade of ``B'' or better.  The {\em meaning} of the value reported may vary with the wealth of the school district of the applicant: a wealthy high school may offer a wide range of AP classes, while an economically disadvantaged school may offer only a handful or even none.  More broadly, in ``Talent is Everywhere,'' SP Danielle Allen has proposes a method of college admission decision-making based on the belief that talented students are geographically distributed.  In analogy, we expect that ``variability is everywhere,'' in the sense that both talent and lack of talent are distributed among different demographic groups.  The data must contain features sufficient for capturing this variability.  

Assuming that variability is present in a set $S$, we should demand such variability in any fair predictor.  A collection ${\cal C}$ of sets in a multi-calibrated predictor also provides characterizations of individuals who may be comparable for the scoring task at hand.  Thus, we are concerned with the question of evaluating the collection ${\cal C}$ given the features in the data: A scoring function that distinguishes talented students from untalented students in one demographic group but not in others is underserving the latter populations.  Unfortunately, multi-calibration with respect to ${\cal C}$ does not ensure anything relevant about the properties of ${\em C}$.  To this end, co-PI Dwork and collaborators have recently suggested the notion of {\em latitude}~\cite{DKRRY19}, which captures the extent to which ${\em C}$ (and the training data) pin down the outcomes for a set~$S \in {\cal C}$.  Since that work was written, co-PI Dwork and her co-authors have been studying this notion, with the goal of obtaining actionable desiderata for scoring functions that capture these concerns.  

Finally, the accuracy criteria require the scoring functions to capture the world as it is, in which people are routinely disadvantaged and degraded based on immutable and irrelevant traits.  There is no guidance on how and when to adjust scores to reflect an ideal world, in which each individual is supported to reach her full potential.  Even stating the goal is a major challenge, but this is precisely the kind of question the interdisciplinary strength of the proposed Institute will help us to attack.
%
% An interesting question is whether we can bring to bear the techniques of Daskalakis {\it et al.} on estimating efficient statistics from truncated samples~\cite{DGTZ18}.
%https://arxiv.org/pdf/1809.03986.pdf



Another basic issue confronting notions of individual fairness is how to interpret probabilities. The outputs of {\em risk assessment tools}, or {\em scoring functions}, are often described as probabilities: What is the probability that the tumor $T$ will metastasize under a given course of treatment?  What is the probability that this individual will click on an ad, or commit a violent crime?
But what does ``probability'' mean for a non-repeatable event?  For example, suppose we have two studies of tumors.  One study examines tumors with specific genetic markers and reports that $40\%$ of these metastasize.  The second study examines tumors with other markers and reports that $70\%$ metastasize.  Suppose the tumor $T$ shares the characteristics of both studies.  What should we conclude: $40\%$ or $70\%$?  Or perhaps neither: what if the second study also has a metastasis rate of $40\%$?  %Should we interpret this as both studies telling us that $40\%$ is the right answer, or should we interpret this as reflecting elevated risk, as $T$ has two sets of risk factors?  Finally, if some tumors with the characteristics of the first ($40\%$) study also share the characteristics of the second ($70\%$) study, but $T$ does not, then in the $40/70$ case should we conclude that the risk for $T$ is {\em less than} $40\%$?  

Concluding {\em individual} risks from statistical information about groups is tricky (at best!), and yet AI is routinely called upon to perform such deductions. When fairness is concerned, the question of ``why did you view me as part of this group rather than another, less risky, group?" is especially critical. At a minimum, when performing individual predictions, we should be able to understand their meaning and their guarantees in terms of the potential for unfair discrimination.
%We discuss here the approach of the proposed research towards this crucial and ambitious objective.

The search for a rigorous approach to individual probabilities dates back at least as far as the early 1980s. Indeed, in his recent survey paper ``On Individual Risk,'' Philip Dawid examines nine explications of the term ``individual risk'' based on a variety of interpretations of ``probability.''
(Dwork will co-teach a graduate reading course with Prof.\,Joseph Blitzstein, from the Harvard Statistics department, on the literature on individual probabilities in Fall, 2020.) Co-PI Dwork and collaborators have proposed viewing individual risk through the lens of complexity theoretic-randomness, drawing an analogy between the sets used in multi-calibration and statistical tests used in the theory of pseudo-randomness.  This Institute will support continued research in this direction.

In~\cite{DKRRY19} Co-PI Dwork and collaborators generalized the multi-set approach to fairness in~\cite{KNRR18,HKRR18} to define definitions of fairness for {\em ranking} individuals. As in multi-calibration, where the task is to learn to assign real-valued {\em scores} to individuals based on training data with only {\em binary} labels, the ranking algorithms of Dwork {\it et al.} rely only on training data with binary outcomes: no examples of real-valued scores are given to the training algorithm.  Rankings introduce unique challenges, as fairly ranking an individual (or even considering average rankings for members of a specific demographic group) requires understanding their qualities and qualifications in relation to those of others. In~\cite{DKRRY19} Co-PI Dwork and her collaborators investigated ``Occam's razor'' conditions that allow the learning of accurate ranking functions, as well as (1) fairness requirements based on historical binary outcomes training data, and (2) fairness requirements based on a ``catalog of evils'' describing poor relative treatment of groups. She and her coauthors showed that, in their respective strongest forms, these two seemingly unrelated flavors of conditions in (1) and (2) are equivalent. 

Despite the explosion of research in algorithmic fairness and the many directions set out in this proposal, there remains much foundational work to be done.  Even if we cannot find satisfying, actionable definitions for very wide settings, there may be more restricted settings (like the many-problem setting of \cite{KRS19}) that are amenable to meaningful, special-purpose definitions. 

%How can we design automated systems that will do appropriate exploration in order to provide robust performance in changing environments?
%\\
%Basic research on definitions of "fairness", "equal treatment", "disparate impact". (Involves both aggregate statistical notions, and individual-level notions, as well as hybrids of the two that operate at other levels of abstraction).

The original notion of individual metric fairness proposed by co-PI Dwork and collaborators may be more actionable than we thought: Combining insights from the field of human-computer interaction (HCI) and learning theory, Co-PI Dwork's student Christina Ilvento showed how to obtain an approximation of a metric from a human arbiter, who may have an excellent understanding of the degree of (dis)similarity, for a given classification task, between pairs individuals but cannot articulate an algorithm~\cite{Ilvento}.  Ilvento distinguishes between two types of queries to the arbiter: difficult queries ask for absolute distances between individuals, while easy queries ask which of two individuals is closer to a third. Under very mild assumptions Ilvento's method requires only a constant number of difficult queries and $O(n \log n)$ easy queries, where $n$ is the number of individuals in the universe.  A natural question is how to partition the queries among multiple arbiters, each of which may be  knowledgeable about different subpopulations.  This is the subject of an undergraduate research project supervised by Co-PI Dwork.  

Finally, most research on fairness treats the "one-shot" case.  Dwork and Ilvento have shown that in individual and group fairness can behave very badly under composition~\cite{DworkIlvento}.  Recently, together with another collaborator, they have investigated individual and group fairness definitions and solutions for {\em pipelines}.  Pipelines differ from ordinary sequential composition in that individuals may drop out of consideration at any stage~\cite{DIJ20}.  We show that naive auditing is unable to uncover systematic unfairness and that, in order to ensure fairness, some form of dependence must exist between the design of algorithms at different stages in the pipeline. 

Suppose a company selects a team, or {\em cohort}, of individuals to work on an exciting new flagship project and subsequently promotes the highest performer on the team to a leadership position.\footnote{Necessarily some individuals will not be selected for the team, capturing that ``dropping out,'' for example, of the STEM pipeline, is not entirely voluntary.} Although the team selection may be fair in the sense that similarly qualified candidates have similar chances of being chosen for the team, the selection of the highest performer critically depends on the \textit{other members of the team}.  However, being compared fairly to other members of the cohort simply doesn't imply fairness of the entire pipeline, as the competitive landscape can vary between similar individuals.  
Indeed, a fair cohort selection mechanism~\cite{DI2018} 
can exploit the myopic nature of the promotion stage to skew overall fairness.  This can happen either through good intentions ({\it e.g.}, choosing teams so that members of a minority group always have a mentor on the team) or malice (\textit{e.g.}, ensuring that minority candidates are almost always paired with a more qualified majority candidate): in both these cases minorities suffer significantly reduced chances of promotion.

Many questions remain open; in some of these it is not even clear how to \texit{define} fairness.  For example: (1) \cite{DIJ20} does not take into account the preferences of individuals during the team formation process;
(2) Cohorts may interact in the future, {\it e.g.}, the top person from each team is promoted to management, among whom executives are chosen; 
(3) \cite{DIJ20} show that there must be some form of communication from later stages of the pipeline to earlier ones in order for the pipeline to be fair as a whole (those forming the teams must know something about the company policy regarding how bonuses are awarded), but a more formal and thorough treatment of the communication complexity between stages remains open; (4) \cite{DIJ20} show efficient team formation mechanisms for three rich classes of scoring functions that ensure that the entire pipeline is fair, leaving open the problem of characterizing families of scoring functions for which this is possible; and (5) the model in~\cite{DIJ20} considers hiring decisions from a single recruitment cycle, in which a team is formed from a collection of candidates, and does not take into account teams formed over time, say, in which new members are added in subsequent hiring cycles.

\paragraph{ML and Fairness in Criminal Justice}
\cd{This section needs text about the BKC dataset.}


\begin{figure}[h]
\label{fig:risk}
\includegraphics[scale=0.35]{left.png}
\includegraphics[scale=0.35]{right.png}
\caption{Screenshot of comparative risk assessment tool developed as part of Penn's AlgoWatch Initiative; see text for details.}
\end{figure}

Another important dimension of our efforts will be focused on {\em auditing} and comparing deployed predictive models in various ways. This complements more design-oriented algorithmic work, and is important because it can sometimes be conducted unilaterally by an outside observer of an algorithm or model, regardless of the intentions of its designer. Such efforts have been part of initial work on Penn's Algowatch Initiative, whose principals include PI Kearns and SPs Kristian Lum, Christopher Yoo (Penn Law) and Ezekiel Dixon-Roman (Penn Social Policy and Practice). This initiative has received seed funding from the Deans of Engineering, the Law School, and the School for Social Policy and Practice, as well as the Provost's office at Penn; we anticipate that impact of this seed funding will be greatly amplified by the proposed Institute.

An early focus has been on the comparative auditing of deployed predictive models for criminal justice applications. Through a combination of detailed descriptions of the models, their underlying training datasets, and professional contacts of SP Kristian Lum, we have faithfully reconstructed and implemented the following predictive models:

\begin{itemize}
\item {\em Public Safety Assessment (PSA)}: ``The PSA uses nine factors to predict a person’s likelihood of success while on pretrial release. The factors include the person’s current age, prior     convictions, pending charges, and prior failures to appear in court pretrial. The PSA generates a score ranging from 1 to 6 on two separate scales – new criminal activity (i.e., arrest) and     failure to appear in court.''
% The assessment may also generate a flag to indicate whether a person presents 
% an elevated likelihood of being arrested for a new violent crime if released during the pretrial period.''
\footnote{See \url{https://www.psapretrial.org/}}
\item {\em Virginia Pretrial Risk Assessment Instrument (VPRAI)}: ``A Virginia Pretrial Risk Assessment Instrument (VPRAI) examines a
    defendant’s status at the time of the arrest related to any active community
    criminal justice supervision, current charges, pending charges, criminal
    history, history of failure to appear, history of violent convictions,
    employment, and history of drug abuse.''
    % For this reason, the instrument is
   %  primarily intended to be completed after arrest and presented at the first
    % court appearance.''
\footnote{See \url{https://www.dcjs.virginia.gov/sites/dcjs.virginia.gov/files/publications/corrections/virginia-pretrial-risk-assessment-instrument-vprai_0.pdf}}
\item {\em Ohio Risk Assessment System (ORAS)}:``The Ohio Risk Assessment System (ORAS) is a statewide assessment system 
    that specifically provides risk assessment instruments at pretrial, community supervision, prison intake, and community reentry.''
    % Validation results reveal that all assessment instruments can significantly distinguish between risk levels.''
    \footnote{See \url{http://www.kscourts.org/Court-Administration/Pretrial_Justice_Task_Force/files/Latessa_slides_Dec_2018.pdf}}
\item {\em New York City Criminal Justice Agency Risk Assessment Tool (CJA)}: ``CJA administers New York City’s release assessment to 
    nearly every individual arrested and held for arraignment. The assessment evaluates the likelihood that an individual released before trial will return for court appearances.''
    % Using extensive New York City data, with independent experts and extensive feedback from court actors and the community, CJA has updated the release assessment to provide judges a % % more fair and accurate pretrial decision making aid.''
    \footnote{See \url{https://www.nycja.org/release-assessment}}
\end{itemize}

In addition to these deployed and actively used risk assessment models, we have also implemented a number of models learned from survey data gathered from Penn undergraduates taking last year's pilot ``Science of Data Ethics'' course (being taught this year
by PI Kearns and SP Lum),
as part of a controlled study on subjective notions of fairness. This survey data elicits pairwise similarity
assessments from COMPAS criminal recidivism records, and uses fair ML methods developed by PI Kearns,
co-PI Roth and colleagues \cite{JKNRSW19} to learn predictive models constrained by the subjective fairness assessments.
This permits comparison between the models developed and deployed by actual criminal justice agencies, and the intuitive fairness notions elicited from the survey subjects.

One of the research challenges in making comparisons between such risk assessment tools and models is the fact that each of them may use different features and inputs, and even shared features may have meaningfully different interpretations and definitions. Our basic methodology has been to rectify shared features by careful examination of the underlying definitions and data when possible. We can then use pairwise correlations from available datasets (e.g. the COMPAS criminal recidivism dataset) and simple independence assumptions to design an overall generative model
or distribution over the union of all features used by all the models.

We have implemented such a generative model and the four deployed models and subjective fairness in a graphical comparative risk assessment tool visualized in Figure~\ref{fig:risk}. In the tool, the user can either fill in values for all of the features needed by the collection of models, or they may use the "generate" functionality to draw correlated values from the underlying generative model. Each input feature is labeled by which of predictive models described above use it (e.g. "VPRAI", "CJA" etc.; ``AW'' refers to the subjective fairness models
as part of the AlgoWatch Initiative), and at the bottom of the GUI the risk assessments of the various models are shown. This tool permits easily visualization of differences between the models generally, and on particular inputs. For instance, in the example shown, the PSA and CJA models differ significantly in their assessment of the likelihood that the individual in question will fail to appear for a mandated court appearance, with the PSA model predicting its maximum risk level possible and the CJA predicting on the lower end of its risk range. Importantly, such examples highlight the fact that across national jurisdictions, actually deployed models may be leading to starkly different outcomes (e.g. in the granting or terms of bail) not just in the aggregate, but on specific individuals. We also see notable
differences both within the survey subject models and between them and the deployed models.

The Institute will enable similar research and practical tool development of a much greater scale and scope. Potential projects and topics include:

\begin{itemize}
\item The study of correlations between the outputs of different risk assessment models on increasingly realistic generative models developed from larger and richer datasets. This would permit us to explore and document systematic
        	statistical similarities and differences in risk assessment modeling and outcomes across jurisdictions, which in turn enables awareness and understanding of potential
            injustices and remedies.
\item The development of similar comparative and stand-alone auditing in other application domains, such as lending or consumer credit (which      will be greatly aided by our
 		collaboration with the Philly Fed and their rich consumer finance datasets), or in online advertising (see related discussion in the Policy and Regulatory section XXX).
\item More ideas here..
\end{itemize}

\paragraph{Proposed work with the First Judicial District of Pennsylvania}

\mk{I'm dropping in text Kristian wrote about collaboration with FJD. It's far from clear we'll get through their approval process
in time for the proposal, so we may end up dropping/deleting, but want to have it here as a placeholder for now}

As part of the proposed work on trustworthy AI, we will collaborate with the First Judicial District of Pennsylvania (FJD) on technical, legal, and policy research that is pertinent to the development and implementation of AI models for criminal justice applications in Philadelphia. Though the parameters of this collaboration will evolve to fit the specific cases for which AI-based tools are developed in Philadelphia and the changing laws and policies governing them, we anticipate the following general structure to the collaboration.

We will work with representatives of the FJD to identify areas in the criminal justice system where AI-based tools are being considered, developed, or adopted. We will work closely with the FJD to understand the needs and concerns that are particular to the context--- which notions of fairness are most pertinent? What are the particular policy constraints under which the technology is developed? What are the open policy or legal questions related to the development of AI in criminal justice in Philadelphia? What are the resource constraints under which AI is developed and deployed in Philadelphia? Based on these conversations, our research team will develop new machine learning or statistical methodology that directly addresses the fairness concerns and policy constraints specific to the FJD and Philadelphia. In cases where an AI-based tool is already in use, we will develop an analysis plan to address questions relevant to the FJD pertaining to the impacts of the tool in the real world. These may include questions such as: Is the use of the tool leading to racial disparities in the criminal justice system? Is the tool changing judicial decision-making? How have relevant statistics from the criminal justice system in Philadelphia changed as a result of adopting the AI-based system?

We will work with FJD to determine what data is required to conduct the research. Under appropriate data sharing agreements, FJD will provide the necessary data to test the new methods or evaluate the impact of existing tools. In some cases, if FJD determines the data is too sensitive to share, the research team will provide FJD with computer code they can run on their own data and only report back results. FJD may also only provide the researchers with coarse descriptions of the data, such as which fields it contains, possible values in those fields, and the size of the data for such extreme cases. 

As a specific example, one likely area of collaboration is around the development and evaluation of a new pre-trial risk assessment tool for Philadelphia. Such tools are commonly used to predict future criminal activity during the pre-trial period.  The research team would learn from the FJD about the specific fairness, political, and legal requirements constraining the development of such a tool in Philadelphia and work to design new AI-based methods tailored to these constraints. The research team may also be involved in evaluating the development of other tools designed under such constraints. Should the tool be put into use, we would work with the FJD to analyze the impact of the tool along metrics that are important to the FJD. 




.



%\subsubsection{Economic Foundations of Fairness Constraints}
%{ \acomment Aaron: Adding some text here, not integrated with the previous for now. Likely too long and overly specific}
%The field of algorithmic fairness has yet to settle on definitions; in fact, we have known since the work of \cite{KMR16} and \cite{Chou17} that there are multiple notions of statistical fairness that are all individually reasonable, but mutually incompatible. For example, if we believe that it is the errors of a classifier that lead to harm, we may want to equalize false positive rates and false negative rates across multiple population groups. Or, if we believe that it is important that the actionable content of a prediction be independent of an individual's group, we may want to equalize positive predictive value across groups. But we cannot generally equalize all three \cite{KMR16,Chou17}. This has led to a debate about which --- if any --- of these notions is appropriate to use in particular circumstances. An especially salient use case is criminal recidivism prediction, in which typically ``risk scores'' are computed to estimate the probability that an individual will commit a crime again in the next 18 months if released parole, and parole recommendations are made on the basis of some threshold applied to individual risk scores. Equalizing false positive and false negative rates in particular is a solution that has been criticized in this context because it usually requires \emph{disparate treatment}, in the sense that to achieve it, one must apply a \emph{different threshold} to individual risk scores for different groups. Indeed, simply applying the \emph{same} threshold to each individual (common practice currently) has been proposed as an important aspect of fairness \cite{CPFGH17}. These debates, however, have typically taken place imagining that the world is static, in the sense that policy decisions made will have no effect on the world in which a classifier is being deployed.

%We propose to instead apply game theoretic modeling to endogenize changes in behavior in response to policy changes, and to use the resulting models to study the equilibrium effects of imposing various fairness constraints.

%In preliminary work, we (PIs Roth and Vohra, together with collaborators Mallesh Pai, Sampath Kannan, Chris Jung, and Changwha Lee) have studied the following simple model which we describe here in the context of criminal justice, but is more general: there are two distinct populations of individuals $A$ and $B$. Each individual will eventually face a decision about whether to commit a crime $(C)$ or not $(N)$, which they will make by weighing the value of an \emph{outside option} $v_i$ with the value of crime $v_C$, together with the risk of being punished. The two populations differ only in their distribution of outside options: each individual $i$ draws an outside option value $v_i \sim D_A$ if they are from group $A$, and otherwise draws a value $v_i \sim D_B$. After each individual $i$ decides on whether to commit a crime or not, a noisy signal is produced according to one of two real valued distributions: if they do not commit the crime, the signal is drawn from $s_i \sim S_N$; otherwise it is drawn from $s_i \sim S_C$. The signal distributions are identical for the two populations conditional on the decision of whether to commit a crime or not. They can be arbitrary, but it is useful to imagine that $S_C$ stochastically dominates $S_N$ (and so high signals are more likely for people who have committed crimes). A criminal justice policy will correspond to setting a pair of thresholds $T_A,T_B$ --- one for each population. Individuals from population $A$ will be punished (i.e. jailed) if $s_i \geq T_A$. Individuals from population $B$ will be punished if $s_i \geq T_B$. The thresholds can be set to be equal, but need not be. Once thresholds are fixed, this deterimines false positive $(FP(T))$ and false negative $(FN(T))$ rates for each population (i.e. the chance of being jailed if one does not commit a crime, and the chance of being freed if one does). Given a fixed cost $C$ for being punished, this determines expected utilities for each decision: individuals $i$ from group $g$ will choose to commit crimes exactly when $v_i - FP(T_g)\cdot C \leq v_C - (1-FN(T_g))\cdot C$. Finally, these individual decisions, together with the distributions on outside options $D_A$ and $D_B$ determine a crime rate in each population. A natural objective is that we should want to set thresholds $T_A$ and $T_B$ so as to minimize the overall crime rate.

%Crime rates establish a \emph{prior probability distribution} on the event that an individual $i$ from a particular group $g$ has committed a crime. Once their signal $s_i$ has been observed, this can be updated to a posterior belief that they have committed the crime. This posterior belief is what corresponds to \emph{risk scores}, and a solution that equalizes positive predictive value across populations should set equal thresholds on posterior beliefs, which will generally correspond to \emph{different} thresholds $T_A$ and $T_B$ on the raw signals (because the outside option distributions are different, and hence so are the crime rates/prior distributions). We refer to this as the myopic solution since the welfare maximizing solution has this form when one ignores the equilibrium effect that policy has on crime rates \cite{CPFGH17}. On the other hand, the solution that equalizes false positive and false negative rates will set equal thresholds $T_A=T_B$ on the raw signals, which will generally correspond to \emph{different} thresholds on the posterior beliefs/risk scores. We have shown that in this setting, the solution that minimizes crime rates is always the one that corresponds to setting differential risk-score thresholds so as to equalize false positive rates! In particular, the crime-rate minimizing solution will typically have different positive predictive value across populations. In terms of a policy pronouncement, this corresponds to committing \emph{not to condition on group membership when computing risk scores}, even when group membership is statistically informative. This is because conditioning on information that an individual has no ability to change (group membership) has a perverse effect on incentives to commit crime. This is how it differs from the myopic solution, which conditions on all available information.

%Going forward, we hope to generalize this result so as to be able to give more robust guidance in a wider range of circumstances. In particular, our current setup is limited to the setting in which 1) signal distributions are identical across populations conditional on the decision to commit a crime, and 2) signal distributions are independent of outside option values, conditional on the decision to commit a crime. Neither of these conditions is fully met in practice. We will investigate whether there are general, weak conditions under which the optimal solution has a false positive rate differential that is \emph{smaller} than the myopic solution. We will also investigate richer models, in which detection rates are a function of the decisions of individual police officers, who may have their own incentives that need to be managed. Finally, we will investigate this framework as it relates to individual notions of fairness \cite{awareness,JKMR16,KNRW18,HKRR18,GJKR18,KRS19,JKNRSW19}.







==> sections/model.tex <==
In this section, we introduce the necessary background for individual fairness and the cohort selection problem, give motivating examples to illustrate the nuances of cohort-based pipelines and convert the intuition behind these examples into formal definitions for robustness in cohort-based pipelines.

\subsection{Preliminaries}
We base our model on individual fairness, as proposed in \cite{dwork2012fairness}. The intuition behind individual fairness is that ``similar individuals should be treated similarly.''
What constitutes similarity for a particular classification task is assumed to be provided as a metric which captures society's best understanding of who is similar to whom in the classification context.
%where similarity is encoded in a task specific metric.
%The metric is intended to capture society's best understanding of who is similar to whom in a particular task setting, e.g., college admissions.
In this work, we will assume the metric is given. Below we formally define individual fairness as in \cite{dwork2012fairness} with a natural Lipschitz relaxation.
\begin{definition}[$\alpha$-Individual Fairness  \cite{dwork2012fairness}]\label{def:individualfairness} Given a universe of individuals $U$, and a metric $\D: U \times U \rightarrow [0,1]$ for a classification task with outcome set $O$, a randomized classifier $C: U \rightarrow \Delta(O)$ (can be viewed as the ordered set $\left( C(u)\right)_{u \in U}$), and a distance metric $d:\Delta(O) \times \Delta(O) \rightarrow [0,1]$ over distributions over outcomes, $\left(C(u)\right)_{u \in U}$ is
$\alpha-$\textit{individually fair}
if and only if for all $u,v \in U$, $d(C(u),C(v)) \le \alpha \D(u,v)$.
\end{definition}
\noindent Individual fairness is a strong definition compared to others proposed in the literature, and although it is based on fairness constraints for individuals it is also a powerful tool for uncovering systemic discrimination.\footnote{Critically, it does not have the composition inconsistency problems of group or statistical definitions of fairness. See \cite{DI2018} for more details.}
Individual fairness was originally proposed in the context of independent classification, i.e. each individual is classified exactly once, independently of all others. However, in many practical settings individuals cannot be classified independently, particularly when there are a limited number of positive classifications available (e.g. a university which can only accept a limited number of students each year, an advertiser with a limited budget).
Dwork and Ilvento formalized this problem as the ``cohort selection problem,'' in which a set of exactly $n$ individuals must be selected such that the probabilities of selection conform to individual fairness constraints \cite{DI2018}.
\begin{definition}[Cohort Selection Problem \cite{DI2018}]\label{def:basiccohort}
Given a universe $U$, an integer $n$ and a task with metric $\D$, select a set of exactly $n$ individuals such that the probability of selection is 1-Lipschitz with respect to $\D$, where the probability of selection is taken over all randomness in the system. We call a mechanism that satisfies these criteria an \textit{individually fair cohort selection mechanism}.
\end{definition}

\subsection{Model and motivating examples}
Throughout this work, we consider a stylized pipeline model of cohort selection followed by scoring in the context of the cohort. More formally, given a set of permissible cohorts $\mathcal{C}$ (e.g. cohorts of size  $n$), first a cohort is chosen by a cohort selection mechanism $\Mech$, and then a scoring function $f: \mathcal{C} \times U \rightarrow [0,1]$ assigns a score to each member of the cohort ($f(C,x) := 0$ for $x \notin C$).  We primarily consider pipelines with a single cohort selection step followed by a scoring step, but our results generalize (with some  important exceptions) to multiple selection or scoring steps, which we discuss in  Appendix \ref{appendix:generalizingmultiplecohortselectionsteps}.
For ease of notation, we associate a probability distribution $\DistMech$ over $\mathcal{C}$ with $\Mech$, such that $\DistMech(C)$ is the probability that $\Mech$ outputs a particular $C \in \mathcal{C}$.
Notice that the probability that $\Mech$ selects a particular individual $u\in U$ maybe split between different cohorts. We denote the set of cohorts containing $u$ as $\mathcal{C}_u$, and the probability that $\Mech$ selects $u$ can be expressed $p(u)=\sum_{C \in \mathcal{C}_u}\DistMech(C)$.

As initial constraints on $\Mech$ and $f$, we assume that $\Mech$ is an individually fair cohort selection mechanism and that $f$ is individually fair within the cohort it observes, i.e., it is \textit{intra-cohort individually fair}: %(Note that $f$ may be designed at a later point in time by different individuals than the designers of $\Mech$, so it's not reasonable for $f$ to maintain the full context of $\Mech$ and $U$.)
%More formally, we define \textit{intra-cohort individual fairness:}
\begin{definition}[Intra-cohort individual fairness] Given a cohort $C$, a scoring function
 $f:\mathcal{C}\times U \rightarrow [0,1]$ is \textit{intra-cohort individually fair} if for all $C \in \mathcal{C}$, $\D(u,v) \ge |f(C, u) - f(C,v)|$ for all $u, v \in C$. %\in \mathcal{C}$.
\end{definition}
\noindent Although $f$ is constrained \textit{within} a particular cohort, $f(C_1, u)$ can be different from $f(C_2, u)$ if $C_1 \neq C_2$. We will often refer to an individual $u$ appearing in a ``cohort context'' to discuss how the cohort apart from $u$ impacts the treatment of $u$ or how swapping $u$ for a different individual $v$ changes outcomes. We use $\Context{C}\cup\{ u\}$ and $\Context{C} \cup \{v\}$ to indicate a context  $\Context{C} \in \{C \backslash \{x\} \mid C \in \mathcal{C}, x \in C \}$, where it is assumed $u,v \notin \Context{C}$.


\subsection{Motivating Examples}
%Given these strict constraints on $\Mech$ and $f$, it would initially seem that the combination of $\Mech$ and $f$ should also satisfy individual fairness. However, as clearly noted in \cite{DI2018}, there is no guarantee of fairness under arbitrary composition, even when all components are individually fair. While the potential for bad interactions between the initial cohort selection and subsequent post-processing is troubling, it is critical to realize that this problem is not merely potential but \textbf{likely} and the resulting unfairness is unbounded.
Given that $\Mech$ and $f$ are both individually fair with respect to the same metric, it would initially seem that composing the two in a pipeline should behave like ``functional composition'' or repeated classification as in \cite{DI2018}, with unfairness only on the order of an increased Lipschitz constant.
However, we show that cohort-based pipelines can result in unbounded unfairness due to the myopic nature of $f$, and that this bad behavior is not merely potential but likely.
To illustrate the ease with which an unwitting (or an actively malicious) system designer can run into trouble, we present the following examples.

%Suppose that the universe consists of three types of individuals $U_h$, individuals highly qualified for a task, $U_m$, individuals with average qualification, and $U_l$, individuals with limited qualification. The metric for the task assigns distances of $\D(u_h,u_m)=0.25$, $\D(u_h,u_l)=0.75$ and $\D(u_m,u_l)=0.5$ for individuals of each type.
\begin{example}\label{example:bonussplitting}
Consider a set of individuals with a range of qualifications applying to join a new project team at a company.
The hiring manager has heard that mutual support and mentorship are very important for minority candidates (having read e.g. \cite{hbr2001}). Therefore they decide to select a team consisting of a random subset of the candidates with average qualifications and either two highly qualified minority candidates or a single highly qualified majority candidate as the team leader(s). This ensures that if a highly qualified minority candidate is chosen they will have mutual support from another highly qualified minority candidate. One year later, the CEO decides to give a bonus to the members of the project team, which will be split proportional to their performance on the team (which is in turn proportional to their original qualification). Notice that although minority and majority leaders had equal probability of being chosen for the team, the minority leaders ``split'' their bonuses, whereas their majority counterparts get the largest share of the bonus to themselves.
\end{example}
\noindent Example \ref{example:bonussplitting} demonstrates two important issues: (1) later stages of the pipeline may be designed by different parties without knowledge of the context of earlier decisions and (2) individually fair policies that are dependent on the cohort chosen can result in arbitrarily different treatment of similar individuals under composition.
However, \textit{proportional} division of bonuses isn't really the problem with Example \ref{example:bonussplitting}, and in fact, \textit{equal} bonus shares can result in similarly bad behavior under composition.
\begin{example}\label{example:steering}
Suppose that the company decides to award bonuses based on the team's overall performance, and each individual receives an equal share of their team's bonus.
Imagine that minority individuals are viewed (rightfully or not) as having higher emotional intelligence and interpersonal skills. When choosing teams for new projects, the core of the team is always chosen in the same way. However, if the project is likely to be frustrating, the company chooses a highly qualified minority candidate as the team leader as they are viewed as being more capable of leadership in a challenging situation. After a few months, only less qualified individuals are willing to remain on the frustrating project teams, and the average qualification of those teams drops. After a year, bonuses are awarded to each individual based on their team's overall performance. Even though each individual within a team gets the same bonus, teams led by minorities have dropped in average qualification, and receive smaller bonuses than their counterparts on teams with majority leaders.
\end{example}
\noindent Example \ref{example:steering} serves as an important counterexample to the common misconception that equal treatment is always individually fair. In fact, the basis for equal treatment may have been polluted by prior decisions or their side effects (e.g. attrition). It's also critical to note that Examples \ref{example:bonussplitting} and \ref{example:steering} can be made more extreme in the case of a malicious pipeline designer, and we provide an extended set of motivating examples, similar to the Catalog of Evils of \cite{dwork2012fairness}, in Appendix \ref{appendix:extendedmotivation}. We also give a simple construction for individually fair cohort selection mechanisms which mask malicious intent in Appendix \ref{appendix:existingmechs}, e.g., explicitly steering minority candidates to specific team types while still maintaining individual fairness with respect to the overall probability of selection.

\subsection{Robustly fair pipelines}
Roughly speaking, the problems with pipelines stem from the fact that later stages in the pipeline behave fairly within the context of the cohort they observe, but the initial cohort selection mechanism \textit{doesn't guarantee that similar individuals have similar probability of appearing in the same cohort context.} One's first thought might be to design $f$ in lockstep with $\Mech$, or to require $f$ to adapt to an arbitrary choice of $\Mech$. Unfortunately, in realistic settings $f$ may be designed at a later point in time by an entirely different set of individuals who have no context for the original choice of $\Mech$. Indeed, later stages in the pipeline may be completely ignorant of the existence of prior stages, e.g. a manager deciding on employee compensation may be unaware of automated resume screening.

We take the view that it is more practical to design the initial cohort selection steps to be robust to composition with a rich family of scoring functions.
For example, the designers of a hiring procedure might not know exactly how compensation will be decided at a later date, but they may know that their company's fundamental operating policies require that similarly qualified individuals receive similar compensation within a particular cohort. Thus, our goal is to formalize what it means to design a hiring procedure that composes fairly with any compensation policy of a particular type, i.e. designing $\Mech$ that is robust to composition with all $f$ in some collection of scoring functions $\F$.
But what exactly does it mean for the composition of the components of a pipeline to be fair? In the one-shot classification setting, the outcome space is clearly specified by a single classifier and the key question is which distance measure over distributions on outcomes to use, e.g. total variation distance. In the case of pipelines, the considerations for individual fairness are more subtle because the outcome space is the union of the outcomes of two separate procedures which may be separated significantly in time. In particular, we must consider two important questions: (1) how does the perception of fairness change conditioned on individuals being selected for the cohort and (2) how does certainty of outcomes affect fairness.
In the remainder of this section, we consider these two questions and frame the notion of robustness parametrized by the two axes: distribution and distance measure over distribution.

%We devote the remainder of this section to formalizing our fairness requirements in considering what it means for similar individuals have similar distributions for pipeline outcomes.

%In particular, we must formalize what it means for similar individuals to have similar distributions over pipeline outcomes, as there are multiple components of the pipeline outcome, i.e. ``selected'' or not and score conditioned on selection.
%There are two axes we must consider: (1) what is the appropriate distribution over outcomes, i.e., conditioned on being selected or not, and (2) how should we measure distances between distributions over outcomes.

\subsubsection{Choosing the distribution}
First, we consider over which distributions to evaluate fairness.
It's critical to account for the fact that any individuals not selected by $\Mech$ never receive a score from $f$, and therefore the relevant outcome space is the union of possible scores and ``not selected,'' i.e. $O_{pipeline}: = [0, 1]\cup \{\notselected\}$. Thus conditioning on whether an individual was selected or not changes the relevant outcome space and, more importantly, changes the \textit{perception} of fairness.
\begin{example}[Perception of conditional probability]\label{example:conditional}
Suppose Alice and Bob are two similarly (but not identically) qualified job candidates. Alice has probability $p(a)$ of being hired and Bob has probability $p(b)$ of being hired. One year after being hired, Alice and Bob are each awarded a bonus such that the difference in their expected unconditioned bonuses over the randomness of the entire pipeline is equal to  $\D(a, b)$. However, conditioned on Alice (or Bob) having been hired, the difference in their bonuses could be much larger than $\D(a,b)$, as $|p(a)f(a)-p(b)f(b)| =\D(a,b) \not \rightarrow f(a)-f(b) \leq \D(a,b)$.
From the perspective of Alice, Bob and their teammates who have limited insight into the original hiring procedure and who likely consider probability of being hired one year prior to be irrelevant to the question of compensation in the present,
%From the perspective of Alice, Bob and their teammates,
this creates the perception that Alice and Bob are being treated much more differently than their true difference in qualification should allow. %because the probability of either being hired is opaque and irrelevant to the question of compensation at a later date.
By using the unconditioned distribution we allow the probability being hired to ``dilute'' the constraint on the treatments conditioned on being hired.
\end{example}
Choosing whether to use the conditional or unconditional distribution boils down to what perception of fairness is  important. In the case of bonuses or promotions being awarded at a much later date than individuals were originally hired, the conditional perception may be particularly important. However, on shorter time frames or in settings where the only outcome that really matters is the final score, the unconditional distribution may be more appropriate (e.g. resume screening immediately followed by interviews).\footnote{Although in this work we consider pipelines with a single relevant metric, the conditional versus unconditional question is critically important when metrics differ between stages of the pipeline. For example, the metric for selecting qualified members of a team may be different than the metric for choosing an individual from the team to be promoted to a management role, as the two stages in the pipeline require different skillsets.}
% save\footnote{We will later show that the constraints imposed by robustness w.r.t the unconditional distribution are weaker than those imposed by the conditional distribution.}
We consider two approaches which capture these different perspectives:
the \textbf{non-conditional distribution} $\UncondDist{\Mech}{f}{u}$, treats the $\notselected$ outcome as a score of $0$
and the \textbf{conditional distribution} $\CondDist{\Mech}{f}{u}$
 conditions on $u$ being selected in the cohort. More formally:

\begin{definition}[Conditional and non-conditional distributions]
Let $\OriginalDist{\Mech}{f}{u} \in \Delta(O_{\text{pipeline}})$ be the distribution over outcomes arising from the pipeline, i.e. $f \circ \Mech$. $\OriginalDist{\Mech}{f}{u}$ places a probability of $1 - p(u)$ on $\notselected$, and  for $s \in [0,1]$, $\OriginalDist{\Mech}{f}{u}$ places a probability of $\sum_{C \in \mathcal{C}} \Pr[f(C,u)=s]A(C)$ on $s$.
  \begin{itemize}[leftmargin=*]
    \item  The \textbf{non-conditional distribution} $\UncondDist{\Mech}{f}{u}$ is identical to $\OriginalDist{\Mech}{f}{u}$ with the exception that it treats the $\notselected$ outcome as if it had score $0$. That is, for $0 < s \le 1$, $\UncondDist{\Mech}{f}{u}$ places a probability of $\sum_{C \in \mathcal{C} }\Pr[ f(C, u) = s] \DistMech(C)$ on $s$; at $s = 0$, $\UncondDist{\Mech}{f}{u}$ has a probability of $1-p(u) + \sum_{C \in \mathcal{C} } \Pr[ f(C, u) = 0]\DistMech(C)$ on $0$.
    \item The  \textbf{conditional distribution} $\CondDist{\Mech}{f}{u}$ has probability $\frac{\sum_{C \in \mathcal{C} }\Pr[ f(C, u) = s]\DistMech(c)}{p(u)}$ for each score $s \in [0,1]$, i.e., it is $\OriginalDist{\Mech}{f}{u}$ conditioned on the positive outcome of $\Mech(C)$.
  \end{itemize}
\end{definition}
For ease of notation we use $d^{cond}(\OriginalDist{\Mech}{f}{u}):=\CondDist{\Mech}{f}{u}$ and $d^{uncond}(\OriginalDist{\Mech}{f}{u}):= \UncondDist{\Mech}{f}{u}$ to refer to these distributions. (In the next section, this notation is highly convenient for expressing the combination of distribution and distance measure over distributions.)
Each of these approaches can be viewed as a method for converting distributions over $O_{pipeline}$ which are unintuitive for the purposes of defining distances between distributions, to a distribution over $[0,1]$, allowing us to more cleanly define distance measures over distributions.

\subsubsection{Distance measures over distributions}
Now that we have enumerated our choices of distributions over $[0,1]$,
we consider which distance measures over these distributions to use. The natural approach would be to use expectation: that is, $\DUncondE(\OriginalDist{\Mech}{f}{u}) := |\mathbb{E}[\UncondDist{\Mech}{f}{u}] - \mathbb{E}[\UncondDist{\Mech}{f}{v}]|$ (resp. $\DCondE(\OriginalDist{\Mech}{f}{u}):=|\mathbb{E}[\CondDist{\Mech}{f}{u}] - \mathbb{E}[[\CondDist{\Mech}{f}{v}]|$). %(Note: we adopt the convention of specifying distance measures over distributions in terms of individuals, with the specific distribution (either conditional or unconditional) and the distance measure over distributions noted in the superscript for ease of notation.)
Difference in expectation generally captures the unfairness in the examples discussed thus far. However, a subtle issue can arise from the \textit{certainty} of outcomes, which requires greater insight into the distribution of scores.
\begin{example}[Certainty of outcomes]\label{example:certainty}
  Consider two individuals, Charlie and Danielle, who are equally qualified.
   Whenever Charlie is hired, he is either hired onto a team in which he is guaranteed promotion, or a team in which he is guaranteed not to be promoted.
  Danielle, on the other hand, is always hired into teams where promotion is uncertain. Even if Charlie and Danielle have equal probability of promotion over the randomness of hiring and promotion, Charlie has significantly higher certainty about his outcome than Danielle does, which better informs his decisions to stay at the company or leave to try to find better opportunities for advancement.\footnote{For example, Charlie may be assigned to either work on the company's flagship product or on code maintenance, whereas Danielle is assigned to work on a risky project with uncertain outcome.}
\end{example}
As Example \ref{example:certainty} illustrates,
 expected score does not entirely capture problems related to the \textit{distribution} of scores rather than the average score. Although total-variation distance is a natural choice for evaluating such distributional differences, it is too strong for this setting, since we do not want perturbations by a small score (i.e. by $\D(u,v)$) to result in a large metric distance.\footnote{For example, if Charlie receives a score of $0.75$ with probability $1$, while Danielle receives a score of $0.75 - \epsilon$ with probability $0.5$ and a score of $0.75 + \epsilon$ with probability $0.5$, then the total variation distance would be $1$, though these outcomes are intuitively very similar.} We introduce the notion of \textit{mass-moving distance} over probability measures which combines total variation distance with earthmover distance to capture the desire for similar distributions over $[0,1]$ with the flexibility to treat similar \textit{scores} as similar.
 %using the fact that there is a natural metric over the outcome space $[0,1]$ induced by $\ell_1$ distance (i.e. difference).
 \begin{definition}[Mass-moving distance]
 \label{def:mmd}
 Let $\gamma_1$ and $\gamma_2$ be probability mass functions over finite sets $\Omega_1 \subseteq [0,1]$ and $\Omega_2 \subseteq [0,1]$, respectively. We define the \textbf{mass-moving distance} $MMD(\gamma_1, \gamma_2)$ as follows. Let $V \subseteq [0,1]$ be the set of real values $v \in [0,1]$ such that there exist probability mass functions $\tilde{\gamma}_1$ and $\tilde{\gamma}_2$ over $[0,1]$ with finite supports where
 \begin{enumerate}[leftmargin=*]
    \item For $i = 1,2$, there is a measurable function $M_i: [0,1] \rightarrow \Delta(\text{Supp}(\tilde{\gamma}_i)) \subseteq [0,1]^{|\text{Supp}(\tilde{\gamma}_i)|}$ such that for $x \in \text{Supp}(\tilde{\gamma}_i), y \in \text{Supp}(M_i(x))$, it is true that $|x - y| \le 0.5 v$ and that $\tilde{\gamma}_i(y) = \int_{[0,1]} (M_i(x))(y) d\gamma_i(x)$.
     %\item The supports of $\tilde{\gamma}_1$  and $\tilde{\gamma}_2$ are both finite.
     \item The total variation distance $v \ge TV(\tilde{\gamma}_1, \tilde{\gamma}_2) :=  \frac{1}{2} \sum_{w \in \Omega} |\tilde{\gamma_1(w) - \tilde{\gamma}_2(w)|$. 
 \end{enumerate}
 Then we let $MMD(\gamma_1, \gamma_2) = \inf V$.
 \end{definition}
\noindent Condition (1) provides a total variation style constraint, but Condition (2) provides the flexibility to ``perturb mass'' by a small distance. Since there is a natural association between finite support probability distributions over $[0,1]$ and finite support probability mass functions over $[0,1]$, Definition \ref{def:mmd} also gives a notion of distance between probability distributions.\footnote{We slightly abuse notation and use $MMD_{\alpha_1, \alpha)2}(\mathcal{X}_1, \mathcal{X}_2)$ for probability distributions $\mathcal{X}_1$ and $\mathcal{X}_2$, to denote $MMD_{\alpha_1, \alpha_2}(\gamma_1, \gamma_2)$ where $\gamma_1$ is the probability mass function associated with $\mathcal{X}_1$ and $\gamma_2$ is the probability mass function associated with $\mathcal{X}_2$.}
Using mass-moving distance, we can now specify the other two distance measures of interest $\DCondMMD(\OriginalDist{\Mech}{f}{u}) := MMD(\CondDist{\Mech}{f}{u}, \CondDist{\Mech}{f}{v}])$ and $\DUncondMMD(\OriginalDist{\Mech}{f}{u}) := MMD(\UncondDist{\Mech}{f}{u}, \UncondDist{\Mech}{f}{v}])$. By evaluating the properties of each combination of distribution and distance measure, we can capture a range of subtle fairness desiderata in pipelines.


\subsection{Formalizing robustness}
Recall our informal notion that a cohort selection mechanism $\Mech$ is robust to a family of scoring functions $\F$ if the composition of $\Mech$ and any $f \in \F$ is individually fair.
We can now formalize robustness
either \textbf{conditional} or \textbf{unconditional} with respect to either \textbf{expected score} or \textbf{mass moving distance} over score distributions.
% For convenience, we explicitly define four distance measures over pipeline outomces capturing the possible combinations of these parameters:
% \begin{enumerate}
%     \item $\DCondE(u,v) = |\E[\CondDist{\Mech}{f}{u}] - \E[\CondDist{\Mech}{f}{v}]|$
%     \item $\DUncondE(u,v) = |\E[\UncondDist{\Mech}{f}{u}] - \E[\UncondDist{\Mech}{f}{v}]|$
%     \item $\DCondMMD(u,v) = MMD(\CondDist{\Mech}{f}{u}, \CondDist{\Mech}{f}{v}])$
%     \item $\DUncondMMD(u,v) = MMD(\UncondDist{\Mech}{f}{u}, \UncondDist{\Mech}{f}{v}])$
% \end{enumerate}
% \noindent which we now use to formally specify our notion of robustness.
% %We now formalize this notion of robustness with two key properties purposely parameterized to express a range of important settings: (1) the distribution over outcomes and (2) the distance measure over distributions.
% %As we will see below, the choice distribution over outcomes, in particular whether to condition on an individual being selected by $\Mech$ is critical for understanding the \textit{perception} of fairness, and the distance measure over distributions is important in cases where \textit{certainty} impacts our understanding of fairness.
\begin{definition}[Robust pipeline fairness]
Given a universe $U$, a metric $\D$, and a pipeline outcome space $O_{pipeline}$, let $\Mech$ be an individually fair cohort-selection mechanism and let $\F$ be a collection of intra-cohort individually fair scoring functions $\mathcal{C} \times U \rightarrow O$. Let $f$ be any function in $\F$ and
%let $\UncondDist{\Mech}{f}{u}$ (resp. $\UncondDist{\Mech}{f}{u}$)
let $d \in \{\DCondE, \DUncondE,$ $ \DCondMMD, \DUncondMMD\}$ denote the distance measure over distribution on outcomes of $f \circ \Mech$ for $u \in U$. %Let $\DCondE(u,v)$ (resp. $\DUncondE(u,v)$) be a distance measure over distributions on outcomes of the pipeline.
We say $\Mech$ is $\alpha$-\textbf{robust w.r.t $\F$} for $d$
 if $d(u,v) \leq \alpha\D(u,v)$ for all $u,v \in U$ and for all $f \in \F$.
\end{definition}

Throughout the rest of this work, we will examine robustness properties in terms of particular settings of $d$.
A natural question to ask is
how the choices of $d$ relate to each other. As one might expect, mass moving distance over score distributions is a stronger condition than expected score, as we show
in Proposition \ref{prop:mmdimpliesexpectedscore}.\footnote{Specifically, we show that if $\gamma_1$ and $\gamma_2$ are probability measures corresponding to distributions $\mathcal{H}_1$ and $\mathcal{H}_2$ and have a $(\alpha_1, \alpha_2)$-mass moving distance of $d$, then $|\mathbb{E}[\mathcal{H}_1] - \mathbb{E}[\mathcal{H}_2]| \le (2\alpha_1 + \alpha_2) d(u,v)$. Interestingly, despite this strengthening, we show in Theorem \ref{thm:necessarydefexpectedscore} that for some classes of score functions, guaranteeing individual fairness w.r.t mass-mover distance fairness is ``equivalent'' to guaranteeing individual fairness w.r.t expected score.} Moreover, we show in Proposition \ref{prop:implicationexpectedscore} that the conditional robustness implies unconditional robustness up to a Lipschitz relaxation.


==> sections/multiplecohortsdetails.tex <==
We now consider the extension of our model to selecting multiple cohorts simultaneously. 
The first option is to run our mechanism many times, which could potentially result in an individual being mapped to many cohorts. We show this directly yields unconditional robustness guarantees for expected score in the following sense: we take an individual's score to be the \textit{sum} of the individual's scores in all cohorts that they are in. For a mechanism $\Mech'$ that selects $T$ cohorts and a score function $f$, this yields a distribution over outcomes, which we take to be $\OriginalDist{\Mech'}{f}{u}$, and then we define $\DUncondE$ analogously to Section \ref{sec:modeldefinitions}. We show the following simple result: 
\begin{lemma}
Let $\DS$ be a distance metric over (context, individual) pairs. Suppose that a cohort selection mechanism $\Mech$ is $\alpha$-robust w.r.t. $\mathcal{F}_{\DS, \alpha}$ for $\DUncondE$. Consider the mechanism $\Mech'$ that runs a cohort-selection mechanism $\Mech$ $T$ times to select $T$ (possibly overlapping) cohorts. Then, $\Mech'$ is $T \cdot \alpha$-robust w.r.t. $\mathcal{F}_{\DS, \alpha}$ for $\DUncondE$ (in the notation discussed above). 
\end{lemma}
\begin{proof}
Observe that the $\mathbb{E}[\UncondDist{\Mech'}{f}{u}]$ (defined using $\OriginalDist{\Mech'}{f}{u}$ as given above) is $T$ times $\mathbb{E}[\UncondDist{\Mech}{f}{u}]$. The result follows. 
\end{proof}

However, in many practical settings, we may want to ensure that an individual is present in at most one cohort. Our next set of results provides extensions of some of our mechanisms in Section \ref{sec:mechanisms} to handle this setting. Our strategy is to select a large cohort and then split it uniformly at random into ``sub-cohorts.'' 

First, we consider extending a monotonic mechanism in this way to achieve \textit{non-conditional} robustness guarantees. 
\begin{lemma}
Suppose that $\Mech$ is a mechanism that is monotone w.r.t swapping mapping for sets of size $k$. Now, suppose that $S$ is a mechanism that uniformly at random splits a set of of size $k$ into cohorts of size $c_1$, $c_2$, $\ldots$, $c_C$ such that $\sum_{i\in [C]}c_i=k$. Then $\Mech \circ S$ selects $C$ cohorts of size $c_1, \ldots, c_C$ and satisfies Notion 1 for the swapping mapping on cohorts of sizes $c_1, \ldots, c_C$. 
\end{lemma}
\begin{proof}
Observe that $\Mech \circ S$ is monotone w.r.t swapping mapping on cohorts of sizes $c_1, \ldots, c_C$, since $\Mech$ is monotone. 
\end{proof}


Notice that this method can also be used for quality-based mechanisms, to achieve both conditional and non-conditional robustness.

\begin{lemma}
Let $\Mech$ be a quality-based mechanism such that (1) $\Mech$ specifies a single canonical set $(c_1,\ldots, c_n)$ of desired quality group membership counts where $\sum_i c_i=k$ and (2) $\Mech$ selects members of the cohort from a particular quality group uniformly at random from the whole quality group. As long as $c_i$ are divisible by $C$, then $\Mech \circ S$, where $S$ splits the cohort output by $\Mech$ into $C$ equally sized cohorts with quality group counts $(c_1/C,\ldots, c_n/C)$, also satisfies $0$-Notion 2 (and $1$-Notion 1).
\end{lemma}
\begin{proof}
We prove the lemma for $0$-Notion 2 by showing that the conditional distribution over outcomes is identical in the case of $\Mech$ and a quality-based mechanism $\Mech'$ (otherwise identical to $\Mech$) that selects a single cohort of size $k/C$. 
Consider an element $u \in U$ that is selected by $\Mech'$ versus $\Mech\circ S$. Notice that the probability that $u $ appears in a particular cohort $ C$ conditioned on being selected is identical between $\Mech'$ and $\Mech \circ S$. Thus the distribution over scores conditioned on selection is identical between $\Mech'$ and $\Mech \circ S$, and as $\Mech'$ satisfies Notion 2, $\Mech \circ S$ also satisfies Notion 2. Notion 1 guarantees follow from Proposition \ref{prop:implicationnotions}.

% We prove the lemma for Notion 1 by showing that the distance in distributions over scores can only decrease compared with the distributions induced by $\Mech'$. Consider the distribution over $O_{pipeline}$ induced by $\Mech'$ versus $\Mech \circ S$. Notice that conditioned on being selected, the distributions are identical. Thus the only difference in the unconditioned distributions is the relative weight on $0$ versus $(0,1]$. Call the weight on $0$ due to the ``not selected'' outcome $w_0$ for $\Mech'$. Notice that redistributing $w_0$ on $[0,1]$ in proportion with the conditional distribution, which is equivalent to $\Mech \circ S$, cannot increase the distance between distributions for either MMD or difference in expected score. 
\end{proof}


